NDC-Scene: Boost Monocular 3D Semantic Scene Completion in Normalized Device Coordinates Space

Monocular 3D Semantic Scene Completion (SSC) has garnered significant attention in recent years due to its potential to predict complex semantics and geometry shapes from a single image, requiring no 3D inputs. In this paper, we identify several critical issues in current state-of-the-art methods, including the Feature Ambiguity of projected 2D features in the ray to the 3D space, the Pose Ambiguity of the 3D convolution, and the Computation Imbalance in the 3D convolution across different depth levels. To address these problems, we devise a novel Normalized Device Coordinates scene completion network (NDC-Scene) that directly extends the 2D feature map to a Normalized Device Coordinates (NDC) space, rather than to the world space directly, through progressive restoration of the dimension of depth with deconvolution operations. Experiment results demonstrate that transferring the majority of computation from the target 3D space to the proposed normalized device coordinates space benefits monocular SSC tasks. Additionally, we design a Depth-Adaptive Dual Decoder to simultaneously upsample and fuse the 2D and 3D feature maps, further improving overall performance. Our extensive experiments confirm that the proposed method consistently outperforms state-of-the-art methods on both outdoor SemanticKITTI and indoor NYUv2 datasets. Our code are available at https://github.com/Jiawei-Yao0812/NDCScene.

==> tables/Result.tex <==
\begin{table*}
	\begin{subtable}{1.0\textwidth}
		\scriptsize
		\setlength{\tabcolsep}{0.0045\linewidth}
		\captionsetup{font=scriptsize}
		\newcommand{\nyuclassfreq}[1]{{~\tiny(\nyufreq{#1}\%)}}  %
		\centering
		\begin{tabular}{l|c|c|c c c c c c c c c c c|c}
			\toprule
			& & SC & \multicolumn{12}{c}{SSC} \\[-0.9em]
			Method
			& Input
			& {IoU}
			& \rotatebox{90}{\parbox{2cm}{\textcolor{ceiling}{$\blacksquare$} ceiling\nyuclassfreq{ceiling}}} 
			& \rotatebox{90}{\textcolor{floor}{$\blacksquare$} floor\nyuclassfreq{floor}}
			& \rotatebox{90}{\textcolor{wall}{$\blacksquare$} wall\nyuclassfreq{wall}} 
			& \rotatebox{90}{\textcolor{window}{$\blacksquare$} window\nyuclassfreq{window}} 
			& \rotatebox{90}{\textcolor{chair}{$\blacksquare$} chair\nyuclassfreq{chair}} 
			& \rotatebox{90}{\textcolor{bed}{$\blacksquare$} bed\nyuclassfreq{bed}} 
			& \rotatebox{90}{\textcolor{sofa}{$\blacksquare$} sofa\nyuclassfreq{sofa}} 
			& \rotatebox{90}{\textcolor{table}{$\blacksquare$} table\nyuclassfreq{table}} 
			& \rotatebox{90}{\textcolor{tvs}{$\blacksquare$} tvs\nyuclassfreq{tvs}} 
			& \rotatebox{90}{\textcolor{furniture}{$\blacksquare$} furniture\nyuclassfreq{furniture}} 
			& \rotatebox{90}{\textcolor{objects}{$\blacksquare$} objects\nyuclassfreq{objects}} 
			& mIoU\\
			\midrule
   
    
			LMSCNet$^\text{rgb}$~\cite{roldao2020lmscnet} & Occ & 33.93 & 4.49 & 88.41 & 4.63 & 0.25 & 3.94 & 32.03 & 15.44 & 6.57 & 0.02 & 14.51 & 4.39 & 15.88 
			\\
\hline
			AICNet$^\text{rgb}$~\cite{li2020anisotropic} & RGB \& Depth & 30.03 & 7.58 & 82.97 & 9.15 & 0.05 & 6.93 & 35.87 & 22.92 & 11.11 & 0.71 & 15.90 & 6.45 & 18.15 
			\\
\hline
			3DSketch$^\text{rgb}$~\cite{chen20203d}& RGB \& TSDF & 38.64 & 8.53 & 90.45&	9.94 & 5.67 & 10.64 & 42.29 & 29.21 & 13.88 & 9.38 & 23.83 & 8.19 & 22.91
			\\
\hline
 %           SSCNet~\cite{song2017semantic} & ${X}^{\text{TSDF}}$ &  \textcolor{blue}{\textbf{55.12}} & \textcolor{blue}{\textbf{15.09}} & \textcolor{blue}{\textbf{94.67}} & \textcolor{blue}{\textbf{24.43}} &  0.00 & 12.64 & 32.07 & 35.03 & 13.04 &  7.79 & 27.11 & 10.14 & 24.70\\
            
			MonoScene~\cite{cao2022monoscene} & RGB & 	42.51 & 8.89 & 93.50 &  12.06 &  12.57 &  13.72 &  48.19 &  36.11 &  15.13 &  15.22 &  27.96 &  12.94 &  26.94\\
            CanoScene(ours) & RGB & \textcolor{blue}{\textbf{44.17}} & \textcolor{blue}{\textbf{12.02}} &	\textcolor{blue}{\textbf{93.51}} &	\textcolor{blue}{\textbf{13.11}} &	\textcolor{blue}{\textbf{13.77}}&	\textcolor{blue}{\textbf{15.83}}&	\textcolor{blue}{\textbf{49.57}}&	\textcolor{blue}{\textbf{39.87}}&	\textcolor{blue}{\textbf{17.17}}&	\textcolor{blue}{\textbf{24.57}}&	\textcolor{blue}{\textbf{31.00}}&	\textcolor{blue}{\textbf{14.96}}&	\textcolor{blue}{\textbf{29.03}} \\ 
			\bottomrule
		\end{tabular}
		\caption{NYUv2} 
		\label{tab:perf_nyu}
	\end{subtable}

\\ \hspace*{\fill} \\
	\begin{subtable}{1.0\textwidth}
		\scriptsize
		\captionsetup{font=scriptsize}
		\setlength{\tabcolsep}{0.004\linewidth}
		\newcommand{\classfreq}[1]{{~\tiny(\semkitfreq{#1}\%)}}  %
		\centering
		\begin{tabular}{l|c|c|c c c c c c c c c c c c c c c c c c c|c}
			\toprule
			& & SC & \multicolumn{20}{c}{SSC} \\
			Method
			& SSC Input
			& {IoU}
			& \rotatebox{90}{\textcolor{road}{$\blacksquare$} road\classfreq{road}} 
			& \rotatebox{90}{\textcolor{sidewalk}{$\blacksquare$} sidewalk\classfreq{sidewalk}}
			& \rotatebox{90}{\textcolor{parking}{$\blacksquare$} parking\classfreq{parking}} 
			& \rotatebox{90}{\textcolor{other-ground}{$\blacksquare$} other-grnd\classfreq{otherground}} 
			& \rotatebox{90}{\textcolor{building}{$\blacksquare$} building\classfreq{building}} 
			& \rotatebox{90}{\textcolor{car}{$\blacksquare$} car\classfreq{car}} 
			& \rotatebox{90}{\textcolor{truck}{$\blacksquare$} truck\classfreq{truck}} 
			& \rotatebox{90}{\textcolor{bicycle}{$\blacksquare$} bicycle\classfreq{bicycle}} 
			& \rotatebox{90}{\textcolor{motorcycle}{$\blacksquare$} motorcycle\classfreq{motorcycle}} 
			& \rotatebox{90}{\textcolor{other-vehicle}{$\blacksquare$} other-veh.\classfreq{othervehicle}} 
			& \rotatebox{90}{\textcolor{vegetation}{$\blacksquare$} vegetation\classfreq{vegetation}} 
			& \rotatebox{90}{\textcolor{trunk}{$\blacksquare$} trunk\classfreq{trunk}} 
			& \rotatebox{90}{\textcolor{terrain}{$\blacksquare$} terrain\classfreq{ &terrain}} 
			& \rotatebox{90}{\textcolor{person}{$\blacksquare$} person\classfreq{person}} 
			& \rotatebox{90}{\textcolor{bicyclist}{$\blacksquare$} bicyclist\classfreq{bicyclist}} 
			& \rotatebox{90}{\textcolor{motorcyclist}{$\blacksquare$} motorcyclist.\classfreq{motorcyclist}} 
			& \rotatebox{90}{\textcolor{fence}{$\blacksquare$} fence\classfreq{fence}} 
			& \rotatebox{90}{\textcolor{pole}{$\blacksquare$} pole\classfreq{pole}} 
			& \rotatebox{90}{\textcolor{traffic-sign}{$\blacksquare$} traf.-sign\classfreq{trafficsign}} 
			& mIoU\\
			\midrule
	
            LMSCNet$^\text{rgb}$~\cite{roldao2020lmscnet} & Occ & 28.61 & 40.68 & 18.22 & 4.38 & 0.00 & 10.31 & 18.33 & 0.00 & 0.00 & 0.00 & 0.00 & 13.66 & 0.02 & 20.54 & 0.00 & 0.00 & 0.00 & 1.21 & 0.00 & 0.00 & 6.70 \\
\hline
            3DSketch$^\text{rgb}$~\cite{chen20203d} & RGB \& TSDF & 33.30 & 41.32 & 21.63 & 0.00 & 0.00 & 14.81 & 18.59 & 0.00 & 0.00 & 0.00 & 0.00 & 19.09 & 0.00 & 26.40 & 0.00 & 0.00 & 0.00 & 0.73 & 0.00 & 0.00 & 7.50  \\
            \hline

            AICNet$^\text{rgb}$~\cite{li2020anisotropic} & RGB \& Depth & 29.59 & 43.55 & 20.55 & 11.97 & 0.07 & 12.94 & 14.71 & 4.53 & 0.00 & 0.00 & 0.00 & 15.37 & 2.90 & 28.71 & 0.00 & 0.00 & 0.00 & 2.52 & 0.06 & 0.00 & 8.31  \\
            
%			*JS3C-Net$^\text{rgb}$~\cite{yan2021sparse}& $\hat{X}^{\text{pts}}$& 34.00 & 47.30 & 21.70 & 19.90 & 2.80 & 12.70 & 20.10 & 0.80 & 0.00 & 0.00 & 4.10 & 14.20 & 3.10 & 12.40 & 0.00 & 0.20 &  0.20 &  8.70 &  1.90 &  0.30 &  8.97  \\

%            SSCNet~\cite{song2017semantic} &$\hat{X}^{\text{TSDF}}$ & 40.93 & 51.28 & 22.38 & 9.07 & 0.02 & 15.20 & 22.32 & 4.69 & 0.00 & 0.00 & 2.43 & 22.24 & 4.33 & \textcolor{blue}{\textbf{31.21}} & 0.00 & 0.01 & 0.00 & 3.57 & 4.83 & 1.49 & 10.27\\
            \hline
			MonoScene~\cite{cao2022monoscene} & RGB &  37.12 & 57.47 & 27.05 & 15.72 & 0.87 & 14.24 & 23.55 & 7.83 & 0.20 & 0.77 & 3.59 & 18.12 & 2.57 & 30.76 & 1.79 & 1.03 & 0.00 & 6.39 & 4.11 & 2.48 & 11.50 \\

 %           Voxformer~\cite{li2023voxformer} & $X^{\text{RGB}}$ & \textcolor{blue}{\textbf{44.02}} & 54.76 & 26.35 & 15.50 & 0.70 & \textcolor{blue}{\textbf{17.65}} & 25.79 & 5.63 & 0.59 & 0.51 & 3.77 & \textcolor{blue}{\textbf{24.39}} & \textcolor{blue}{\textbf{5.08}} & 29.96 & 1.78 & \textcolor{blue}{\textbf{3.32}} & 0.00 & \textcolor{blue}{\textbf{7.64}} & \textcolor{blue}{\textbf{7.11}} & \textcolor{blue}{\textbf{4.18}} & 12.35 \\
            CanoScene(ours) & RGB & \textcolor{blue}{\textbf{37.17}} & \textcolor{blue}{\textbf{59.20}} & \textcolor{blue}{\textbf{28.24}} & \textcolor{blue}{\textbf{21.42}} & \textcolor{blue}{\textbf{1.67}} & \textcolor{blue}{\textbf{14.94}} & \textcolor{blue}{\textbf{26.26}} &  \textcolor{blue}{\textbf{14.75}} & \textcolor{blue}{\textbf{1.67}} & \textcolor{blue}{\textbf{2.37}} & \textcolor{blue}{\textbf{7.73}} & \textcolor{blue}{\textbf{19.09}} & \textcolor{blue}{\textbf{3.51}} & \textcolor{blue}{\textbf{31.04}} & \textcolor{blue}{\textbf{3.60}} & \textcolor{blue}{\textbf{2.74}} & 
            0.00 & \textcolor{blue}{\textbf{6.65}} & \textcolor{blue}{\textbf{4.53}} & \textcolor{blue}{\textbf{2.73}} & \textcolor{blue}{\textbf{12.70}}\\ 
			\bottomrule
		\end{tabular}\\
%		{\scriptsize* Uses pretrained semantic segmentation network.}
		\caption{SemanticKITTI} %(hidden test set)}
		\label{tab:perf_semkitti}
	\end{subtable}
	\caption{\textbf{Quantitative comparsion} against RGB-inferred baselines and the state-of-the-art monocular SSC method on NYUv2~\cite{silberman2012indoor} and SemanticKITTI~\cite{behley2019semantickitti} dataset. Bold numbers represent the best scores. }
	\label{tab:perf}
\end{table*}

==> tables/Vis.tex <==
\begin{figure*}
	\begin{subfigure}{\linewidth}		
		\centering
		\footnotesize
        \captionsetup{font = footnotesize}
		\renewcommand{\arraystretch}{0.0}
		\setlength{\tabcolsep}{0.003\textwidth}
		\newcolumntype{P}[1]{>{\centering\arraybackslash}m{#1}}
		\captionsetup{font=scriptsize}
		\begin{tabular}{P{0.10\textwidth} P{0.115\textwidth} P{0.115\textwidth} P{0.115\textwidth} P{0.115\textwidth} P{0.115\textwidth} P{0.115\textwidth}}
			Input & %LMSCNet$^\text{rgb}$~\cite{roldao2020lmscnet} & 
   AICNet$^\text{rgb}$~\cite{li2020anisotropic} & 3DSketch$^\text{rgb}$~\cite{chen20203d} & MonoScene~\cite{cao2022monoscene} & NDC-Scene\scriptsize{(ours)} & Ground Truth
			\\[-0.1em]
			\includegraphics[width=\linewidth]{figure/nyu_qualitative/NYU0282_0000_2_color.jpg} & 
			\includegraphics[width=\linewidth]{figure/nyu_qualitative/NYU0282_0000_2_aicnet.png} &
			\includegraphics[width=\linewidth]{figure/nyu_qualitative/NYU0282_0000_2_sketch.png} &
			\includegraphics[width=\linewidth]{figure/nyu_qualitative/NYU0282_0000_2_MonoScene.png} &
			\includegraphics[width=\linewidth]{figure/nyu_qualitative/NYU0282_0000_2_CanoScene.png} &
			\includegraphics[width=\linewidth]
            %{figure/nyu_qualitative/NYU1250_0000_2_CanoScene.png} &
		%	\includegraphics[width=\linewidth]
            {figure/nyu_qualitative/NYU0282_0000_2_gt.png} 
   
			\\[-0.3em]
			\includegraphics[width=\linewidth]{figure/nyu_qualitative/NYU0994_0000_2_color.jpg} & 
			\includegraphics[width=\linewidth]{figure/nyu_qualitative/NYU0994_0000_2_aicnet.png} &
			\includegraphics[width=\linewidth]{figure/nyu_qualitative/NYU0994_0000_2_sketch.png} &
			\includegraphics[width=\linewidth]{figure/nyu_qualitative/NYU0994_0000_2_MonoScene.png} &
			\includegraphics[width=\linewidth]{figure/nyu_qualitative/NYU0994_0000_2_CanoScene.png} &
			\includegraphics[width=\linewidth]
            %{figure/nyu_qualitative/NYU0994_0000_2_CanoScene.png} &
		%	\includegraphics[width=\linewidth]
            {figure/nyu_qualitative/NYU0994_0000_2_gt.png}
			\\[-0.3em] 
			\includegraphics[width=\linewidth]{figure/nyu_qualitative/NYU1101_0000_2_color.jpg} & 
			\includegraphics[width=\linewidth]{figure/nyu_qualitative/NYU1101_0000_2_aicnet.png} &
			\includegraphics[width=\linewidth]{figure/nyu_qualitative/NYU1101_0000_2_sketch.png} &
			\includegraphics[width=\linewidth]{figure/nyu_qualitative/NYU1101_0000_2_MonoScene.png} &
			\includegraphics[width=\linewidth]{figure/nyu_qualitative/NYU1101_0000_2_CanoScene.png} &
			\includegraphics[width=\linewidth]
            %{figure/nyu_qualitative/NYU0970_0000_2_CanoScene.png} &
		%	\includegraphics[width=\linewidth]
            {figure/nyu_qualitative/NYU1101_0000_2_gt.png}
			\\
			\multicolumn{6}{c}{
				\scriptsize
				\textcolor{ceiling}{$\blacksquare$}ceiling~
				\textcolor{floor}{$\blacksquare$}floor~
				\textcolor{wall}{$\blacksquare$}wall~
				\textcolor{window}{$\blacksquare$}window~
				\textcolor{chair}{$\blacksquare$}chair~
                    \textcolor{bed}{$\blacksquare$}bed~
				\textcolor{sofa}{$\blacksquare$}sofa~
				\textcolor{table}{$\blacksquare$}table~
				\textcolor{tvs}{$\blacksquare$}tvs~
				\textcolor{furniture}{$\blacksquare$}furniture~
				\textcolor{objects}{$\blacksquare$}objects
			}
		\end{tabular}
		\caption{\textbf{NYUv2\cite{silberman2012indoor} (test set).}\\[0.5em]}
		\label{fig:qualitative_NYU}
	\end{subfigure}
	\begin{subfigure}{\linewidth}	
		\centering
		\newcolumntype{P}[1]{>{\centering\arraybackslash}m{#1}}
		\setlength{\tabcolsep}{0.001\textwidth}
		\renewcommand{\arraystretch}{0.8}
		\footnotesize
		\captionsetup{font=scriptsize}
		\begin{tabular}{P{0.137\textwidth} P{0.137\textwidth} P{0.137\textwidth} P{0.137\textwidth} P{0.137\textwidth} P{0.137\textwidth}P{0.137\textwidth}}		
			Input & %LMSCNet$^\text{rgb}$~\cite{roldao2020lmscnet} & 
   AICNet$^\text{rgb}$~\cite{li2020anisotropic}  & LMSCNet$^\text{rgb}$~\cite{roldao2020lmscnet}  & MonoScene~\cite{cao2022monoscene} & NDC-Scene~\scriptsize{(ours)} & Ground Truth
			\\[-0.1em]
			\includegraphics[width=\linewidth]{figure/kitti_qualitative/001005.png} &  
			\includegraphics[width=\linewidth]
           % {figure/kitti_qualitative/001385_0_lmscnet.png} & 
		%	\includegraphics[width=\linewidth]
            {figure/kitti_qualitative/001005_0_aicnet.png} & 
			\includegraphics[width=\linewidth]{figure/kitti_qualitative/001005_0_lmscnet.png} & 
			\includegraphics[width=\linewidth]{figure/kitti_qualitative/001005_0_MonoScene.pdf} & 
			\includegraphics[width=\linewidth]
            {figure/kitti_qualitative/001005_0_CanoScene.pdf} & 
			\includegraphics[width=\linewidth]
            {figure/kitti_qualitative/001005_0_gt.pdf} 
			\\[-0.6em]
			\includegraphics[width=\linewidth]{figure/kitti_qualitative/000010.png} & 
			\includegraphics[width=\linewidth]{figure/kitti_qualitative/000010_0_aicnet.png} & 
			\includegraphics[width=\linewidth]{figure/kitti_qualitative/000010_0_lmscnet.png} & 
			\includegraphics[width=\linewidth]{figure/kitti_qualitative/000010_0_MonoScene.pdf} & 
			\includegraphics[width=\linewidth]
            {figure/kitti_qualitative/000010_0_CanoScene.pdf} & 
			\includegraphics[width=\linewidth]
            {figure/kitti_qualitative/000010_0_gt.pdf} 
			\\[-0.6em]
			\includegraphics[width=\linewidth]{figure/kitti_qualitative/000465.png} & 
			\includegraphics[width=\linewidth]
         %   {figure/kitti_qualitative/002505_0_lmscnet.png} & 
	%		\includegraphics[width=\linewidth]
            {figure/kitti_qualitative/000465_0_aicnet.png} & 
			\includegraphics[width=\linewidth]{figure/kitti_qualitative/000465_0_lmscnet.png} & 
			\includegraphics[width=\linewidth]{figure/kitti_qualitative/000465_0_MonoScene.pdf} & 
			\includegraphics[width=\linewidth]
            {figure/kitti_qualitative/000465_0_CanoScene.pdf} & 
			\includegraphics[width=\linewidth]
            {figure/kitti_qualitative/000465_0_gt.pdf} 
			\\		
			\multicolumn{6}{c}{
				\scriptsize
				\textcolor{bicycle}{$\blacksquare$}bicycle~
				\textcolor{car}{$\blacksquare$}car~
				\textcolor{motorcycle}{$\blacksquare$}motorcycle~
				\textcolor{truck}{$\blacksquare$}truck~
				\textcolor{other-vehicle}{$\blacksquare$}other vehicle~
				\textcolor{person}{$\blacksquare$}person~
				\textcolor{bicyclist}{$\blacksquare$}bicyclist~
				\textcolor{motorcyclist}{$\blacksquare$}motorcyclist~
				\textcolor{road}{$\blacksquare$}road~
				\textcolor{parking}{$\blacksquare$}parking~}\\
			\multicolumn{6}{c}{
				\scriptsize
				\textcolor{sidewalk}{$\blacksquare$}sidewalk~
				\textcolor{other-ground}{$\blacksquare$}other ground~
				\textcolor{building}{$\blacksquare$}building~
				\textcolor{fence}{$\blacksquare$}fence~
				\textcolor{vegetation}{$\blacksquare$}vegetation~
				\textcolor{trunk}{$\blacksquare$}trunk~
				\textcolor{terrain}{$\blacksquare$}terrain~
				\textcolor{pole}{$\blacksquare$}pole~
				\textcolor{traffic-sign}{$\blacksquare$}traffic sign			
			}
		\end{tabular}		

  \caption{\textbf{SemanticKITTI~\cite{behley2019semantickitti} (val set).}}
		\label{fig:qualitative_kitti}
	\end{subfigure}
        \captionsetup{font = footnotesize}
       
	\caption{\textbf{Qualitative results on~\ NYUv2~\cite{silberman2012indoor} and SemanticKITTI~\cite{behley2019semantickitti}.} From left to right: (a) RGB input, (b) results of AICNet$^\text{rgb}$~\cite{li2020anisotropic}  (c) results of 3DSketch$^\text{rgb}$~\cite{chen20203d}  (d) results of  MonoScene~\cite{cao2022monoscene} (e) ours results. NDC-Scene achieve higher voxel-level accuracy and better semantic predictions on both datasets compared with existing SSC baselines.}
 
	\label{fig:qualitative}
\end{figure*}

==> tables/ablation.tex <==
\begin{table}
	\centering
	\setlength{\tabcolsep}{0.010\linewidth}
	\centering
	\footnotesize
        \captionsetup{font=footnotesize}
	\begin{tabular}{l|cc|cc}
		\toprule
		& \multicolumn{2}{c}{NYUv2} & \multicolumn{2}{c}{SemanticKITTI} \\
		& IoU $\uparrow$ & mIoU $\uparrow$ & IoU $\uparrow$ & mIoU $\uparrow$ \\
		\midrule
		Ours &  \textbf{44.17} & \textbf{29.03}  & \textbf{37.24}  & \textbf{12.70} 	
		\\
        
		CanoScene-FA & 42.96 \textcolor{blue}{(-1.21)} & 27.69 \textcolor{blue}{(-1.34)} & 37.15 \textcolor{blue}{(-0.09)} & 12.03 \textcolor{blue}{(-0.67)}
		\\
		CanoScene-CI & 43.72 \textcolor{blue}{(-0.45)}  & 28.10 \textcolor{blue}{(-0.93)} & 37.20 \textcolor{blue}{(-0.04)} & 12.26 \textcolor{blue}{(-0.44)}
		\\
		CanoScene-NF & 43.52 \textcolor{blue}{(-0.65)} & 28.22 (\textcolor{blue}{-0.81}) & 37.18 \textcolor{blue}{(-0.06)} & 11.22 \textcolor{blue}{(-0.48)}	
  		\\
		MonoScene & 42.51 \textcolor{blue}{(-1.66)} & 26.94 (\textcolor{blue}{-2.09}) & 37.12 \textcolor{blue}{(-0.12)} & 11.50 \textcolor{blue}{(-1.20)}	
%		\\\hline
%		Ours w/o PA($\theta$ = $5^\circ$)  & 40.96 \tiny$\pm$0.28 & 26.34 \tiny$\pm$0.23 & 34.92 \tiny$\pm$0.34 & \underline{11.35} \tiny$\pm$0.22	
%		\\
%  Ours w/o PA($\theta$ = $10^\circ$)  & 40.96 \tiny$\pm$0.28 & 26.34 \tiny$\pm$0.23 & 34.92 \tiny$\pm$0.34 & \underline{11.35} \tiny$\pm$0.22	
%		\\
%  Ours w/o PA($\theta$ = $15^\circ$)  & 40.96 \tiny$\pm$0.28 & 26.34 \tiny$\pm$0.23 & 34.92 \tiny$\pm$0.34 & \underline{11.35} \tiny$\pm$0.22	
		\\
		
		\bottomrule
	\end{tabular}
	\caption{\textbf{Architecture ablation.} Our components boost performance on NYUv2~\cite{silberman2012indoor} and SemanticKITTI~\cite{behley2019semantickitti}.}
	\label{tab:ablation}
\end{table}

==> tables/ablation_method.tex <==
\begin{table}
	\centering
	\setlength{\tabcolsep}{0.015\linewidth}
	\centering
        \captionsetup{font=footnotesize}
	\footnotesize
	\begin{tabular}{l|ccc}
		\toprule
		& \multicolumn{3}{c}{}  \\
		Methods & w/o PA & w/o CI & w/ DA \\
		\midrule
		CanoScene-FA &  \scalebox{0.85}[1]{$\times$}  & \checkmark & \checkmark \\
  
        CanoScene-CI &  \checkmark  & \scalebox{0.85}[1]{$\times$} & \checkmark \\

        CanoScene-NF &  \checkmark  & \checkmark & \scalebox{0.85}[1]{$\times$}\\
        
		CanoScene &  \checkmark  & \checkmark & \checkmark \\
		\bottomrule
	\end{tabular}
	\caption{ Attributes of different variants of CanoScene. \skq{is it possible to merge table 3 and 4?}}
	\label{tab:ablation_attr}
\end{table}
